Roboflow 100: A Rich, Multi-Domain Object Detection Benchmark

The evaluation of object detection models is usually performed by optimizing a single metric, e.g. mAP, on a fixed set of datasets, e.g. Microsoft COCO and Pascal VOC. Due to image retrieval and annotation costs, these datasets consist largely of images found on the web and do not represent many real-life domains that are being modelled in practice, e.g. satellite, microscopic and gaming, making it difficult to assert the degree of generalization learned by the model. We introduce the Roboflow-100 (RF100) consisting of 100 datasets, 7 imagery domains, 224,714 images, and 805 class labels with over 11,170 labelling hours. We derived RF100 from over 90,000 public datasets, 60 million public images that are actively being assembled and labelled by computer vision practitioners in the open on the web application Roboflow Universe. By releasing RF100, we aim to provide a semantically diverse, multi-domain benchmark of datasets to help researchers test their model's generalizability with real-life data. RF100 download and benchmark replication are available on GitHub.

==> tables/datasets-table-semantic.tex <==
\begin{table*}[t]
    % https://tex.stackexchange.com/questions/31672/column-and-row-padding-in-tables
    \setlength{\tabcolsep}{0.5em} % for the horizontal padding
    {\renewcommand{\arraystretch}{1.2}% for the vertical padding
        \centering
        \begin{longtable}{| l l | c c c |}
            \hline
            Category                                  & Sub Category                         &                               & Dataset                 &                          \\
            \hline
            % Aerial
            \multirow{2}{*}{\textit{Aerial}}          & \textit{space}                       & secondary-chains              & cloud-types             &                          \\
            \cline{3-5}
                                                      & \textit{static cameras}              & aerial-spheres                & soccer-players-5fuqs    & weed-crop-aerial         \\
            \cline{3-5}
                                                      & \textit{drones}                      & aerial-cows                   &                         &                          \\
            \hline
            % Video Games
            \multirow{2}{*}{\textit{Video Games}}     &                                      & farcry6-videogame             & csgo-videogame          & avatar-recognition-nuexe \\
                                                      &                                      & halo-infinite-angel-videogame & team-fight-tactics      & robomasters-285km        \\
            \hline
            % Microscopic
            \multirow{5}{*}{\textit{Microscopic}}     & \multirow{3}{*}{\textit{human}}      & stomata-cells                 & bccd-ouzjz              & parasites-1s07h          \\
                                                      &                                      & cells-uyemf                   & 4-fold-defect           & bacteria-ptywi           \\
                                                      &                                      & mitosis-gjs3g                 & phages                  & liver-disease            \\
            \cline{3-5}
                                                      & \textit{plants}                      & cotton-plant-disease          &                         &                          \\
            \cline{3-5}
                                                      & \textit{inanimate}                   & asbestos                      &                         &                          \\
            \hline
            % Underwater
            \multirow{2}{*}{\textit{Underwater}}      &                                      & aquarium-qlnqy                & peixos-fish             & underwater-objects-5v7p8 \\
                                                      &                                      & coral-lwptl                   &                         &                          \\
            \hline
            % Documents
            \multirow{2}{*}{\textit{Documents}}       & \textit{social media}                & tweeter-posts                 & tweeter-profile         &                          \\
            \cline{3-5}
                                                      & \multirow{3}{*}{\textit{structured}} & document-parts                & activity-diagrams-qdobr &                          \\
                                                      &                                      & signatures-xc8up              & paper-parts             & tabular-data-wf9uh       \\
                                                      &                                      & paragraphs-co84b              &                         &                          \\
            \hline
            % Electromagnetic
            \multirow{2}{*}{\textit{Electromagnetic}} & \textit{night vision}                & flir-camera-objects           &                         &                          \\
            \cline{3-5}
                                                      & \textit{thermal}                     & thermal-cheetah-my4dp         &                         &                          \\
            \cline{3-5}
                                                      & \textit{x-ray}                       & x-ray-rheumatology            & acl-x-ray               & bone-fracture-7fylg      \\
            \cline{3-5}
                                                      & \multirow{2}{*}{\textit{mri}}        & abdomen-mri                   & axial-mri               & gynecology-mri           \\
                                                      &                                      & brain-tumor-m2pbp             &                         &                          \\
            \hline
            % Real World}
            \multirow{20}{*}{\textit{Real World}}     & \multirow{4}{*}{\textit{-}}          & smoke                         & soda-bottles            & wine-labels
            \\ & & digits-t2eg6 & valentines-chocolate & peanuts-sd4kf \\
                                                      &                                      & cavity-rs0uf                  & pills-sxdht             & number-ops               \\
                                                      &                                      & coins-1apki                   & people-in-painting      & cell-towers              \\
            \cline{3-5}
                                                      & \textit{indoor}                      & washroom-rf1fa                & furniture-ngpea         &                          \\
            \cline{3-5}
                                                      & \textit{damage}                      & wall-damage                   & corrosion-bi3q3         & cable-damage             \\
            \cline{3-5}
                                                      & \multirow{2}{*}{\textit{vehicles}}   & excavators-czvg9              & road-traffic            & truck-movement           \\
                                                      &                                      & vehicles-q0x2v                &                         &                          \\
            \cline{3-5}
                                                      & \multirow{2}{*}{\textit{safety}}     & smoke-uvylj                   & road-signs-6ih4y        & street-work              \\
                                                      &                                      & construction-safety-gsnvb     & mask-wearing-608pr      & gauge-u2lwv              \\
            \cline{3-5}
                                                      & \multirow{2}{*}{\textit{electronic}} & circuit-elements              & cables-nl42k            & printed-circuit-board    \\
                                                      &                                      & circuit-voltages              &                         &                          \\
            \cline{3-5}
                                                      & \multirow{3}{*}{\textit{animals}}    & animals-ij5d2                 & trail-camera            & fish-market-ggjso        \\
                                                      &                                      & shark-teeth-5atku             & pests-2xlvx             & insects-mytwu            \\
                                                      &                                      & insects-mytwu                 &                         &                          \\
            \cline{3-5}
                                                      & \multirow{2}{*}{\textit{plant}}      & cotton-20xz5                  & apples-fvpl5            & grass-weeds              \\
                                                      &                                      & lettuce-pallets               &                         &                          \\
            \cline{3-5}
                                                      & \textit{geology}                     & sedimentary-features          &                         &                          \\
            \cline{3-5}
                                                      & \textit{boardgames}                  & chess-pieces-mjzgj            & poker-cards-cxcvz       & uno-deck                 \\
            \cline{3-5}
                                                      & \textit{human activities}            & sign-language-sokdr           & hand-gestures-jps7z     &                          \\
            \hline
            \caption{List of datasets for each category and semantic group selected by the Authors.
                \label{table:datasets-semantic} }
        \end{longtable}
    }
\end{table*}

==> tables/metadata-table-realworld.tex <==
\begin{table*}[t]

    \begin{center}
        \setlength{\tabcolsep}{0.5em} % for the horizontal padding
        {\renewcommand{\arraystretch}{1.2}% for the vertical padding
            \begin{tabular}{|| c | c | c | c c c | c c c | c ||}

                \hline

                \multirow{2}{*}{Dataset}                 &
                \multirow{2}{*}{Classes}                 &
                {Labeling}                               &
                                                         &
                {Images}                                 &    &
                {YOLOv5}                                 &
                {YOLOv7}                                 &
                {GLIP}                                   &
                \multirow{2}{*}{Source}

                                                         &    &              & Hours & Train & Valid & Test  & mAP@.50 & mAP@.50 & mAP@.50:.95
                                                         &
                \\ \hline

                Hand Gestures                            & 14 & 0            & 642   & 178   & 94    & 0.995 & 0.994   & 0       & \href{https://app.roboflow.com/roboflow-100/hand-gestures-jps7z/1}{Roboflow}        \\
                Smoke                                    & 1  & 7            & 522   & 148   & 76    & 0.951 & 0.953   & 0.431   & \href{https://app.roboflow.com/roboflow-100/smoke-uvylj/1}{Roboflow}                \\
                Wall Damage                              & 3  & \textit{n/a} & 325   & 96    & 40    & 0.331 & 0.037   & 0.093   & \href{https://app.roboflow.com/roboflow-100/damage-bah7a/1}{Roboflow}               \\
                Corrosion                                & 3  & 186          & 840   & 304   & 105   & 0.786 & 0.71    & 0.003   & \href{https://app.roboflow.com/roboflow-100/corrosion-bi3q3/1}{Roboflow}            \\


                Excavators                               & 3  & 0            & 2244  & 267   & 144   & 0.919 & 0.921   & 0.274   & \href{https://app.roboflow.com/roboflow-100/excavators-czvg9/1}{Roboflow}           \\
                Chess Pieces                             & 13 & \textit{n/a} & 202   & 58    & 29    & 0.987 & 0.987   & 0.017   & \href{https://app.roboflow.com/roboflow-100/chess-pieces-mjzgj/1}{Roboflow}         \\
                Road Signs                               & 21 & 0            & 1376  & 488   & 229   & 0.956 & 0.966   & 0.036   & \href{https://app.roboflow.com/roboflow-100/road-signs-6ih4y/1}{Roboflow}           \\
                Street Work                              & 11 & 2            & 611   & 175   & 87    & 0.492 & 0.531   & 0.148   & \href{https://app.roboflow.com/roboflow-100/street-work/1}{Roboflow}                \\


                Construction Safety                      & 5  & 505          & 997   & 119   & 90    & 0.894 & 0.885   & 0.259   & \href{https://app.roboflow.com/roboflow-100/construction-safety-gsnvb/1}{Roboflow}  \\
                Road Traffic                             & 12 & 816          & 494   & 187   & 133   & 0.604 & 0.634   & 0.147   & \href{https://app.roboflow.com/roboflow-100/vehicles-80lt0/1}{Roboflow}             \\
                Washroom                                 & 10 & 449          & 1885  & 775   & 318   & 0.616 & 0.636   & 0.146   & \href{https://app.roboflow.com/roboflow-100/washroom-rf1fa/1}{Roboflow}             \\
                Circuit Elements                         & 46 & 311          & 672   & 64    & 36    & 0.051 & -       & 0.001   & \href{https://app.roboflow.com/roboflow-100/circuit-elements/1}{Roboflow}           \\
                Mask Wearing                             & 2  & \textit{n/a} & 105   & 29    & 15    & 0.834 & 0.919   & 0.008   & \href{https://app.roboflow.com/roboflow-100/mask-wearing-608pr/1}{Roboflow}         \\


                Cables                                   & 11 & \textit{n/a} & 4816  & 1220  & 794   & 0.697 & 0.706   & 0.01    & \href{https://app.roboflow.com/roboflow-100/cables-nl42k/1}{Roboflow}               \\
                Soda Bottles                             & 6  & 243          & 1547  & 486   & 216   & 0.958 & -       & 0.098   & \href{https://app.roboflow.com/roboflow-100/soda-bottles/1}{Roboflow}               \\
                Truck Movement                           & 7  & 282          & 740   & 215   & 107   & 0.807 & 0.844   & 0.007   & \href{https://app.roboflow.com/roboflow-100/truck-movement/1}{Roboflow}             \\
                Wine Labels                              & 12 & 249          & 3172  & 841   & 630   & 0.607 & 0.679   & 0.045   & \href{https://app.roboflow.com/roboflow-100/wine-labels/1}{Roboflow}                \\
                Digits                                   & 10 & 144          & 2912  & 824   & 367   & 0.986 & 0.987   & 0.003   & \href{https://app.roboflow.com/roboflow-100/digits-t2eg6/1}{Roboflow}               \\


                Vehicles                                 & 12 & 1121         & 2634  & 966   & 458   & 0.461 & 0.475   & 0.029   & \href{https://app.roboflow.com/roboflow-100/vehicles-q0x2v/1}{Roboflow}             \\
                Peanuts                                  & 2  & 212          & 268   & 77    & 42    & 0.995 & 0.997   & 0.358   & \href{https://app.roboflow.com/roboflow-100/peanuts-sd4kf/1}{Roboflow}              \\
                Printed Circuit Board                    & 34 & 311          & 548   & 80    & 44    & 0.25  & -       & 0       & \href{https://app.roboflow.com/roboflow-100/printed-circuit-board/1}{Roboflow}      \\
                Pests                                    & 28 & 188          & 509   & 153   & 55    & 0.211 & 0.002   & 0.004   & \href{https://app.roboflow.com/roboflow-100/pests-2xlvx/1}{Roboflow}                \\
                Cavity                                   & 2  & 165          & 287   & 93    & 38    & 0.755 & 0.783   & 0.029   & \href{https://app.roboflow.com/roboflow-100/cavity-rs0uf/1}{Roboflow}               \\


                Leaf Disease                             & 3  & 143          & 1589  & 616   & 296   & 0.524 & -       & 0.027   & \href{https://app.roboflow.com/roboflow-100/vehicles-q0x2v/1}{Roboflow}             \\
                Marbles                                  & 2  & 133          & 54    & 19    & 32    & 0.995 & 0.99    & 0.03    & \href{https://app.roboflow.com/roboflow-100/peanuts-sd4kf/1}{Roboflow}              \\
                Pills                                    & 8  & \textit{n/a} & 316   & 90    & 45    & 0.983 & 0.948   & 0.194   & \href{https://app.roboflow.com/roboflow-100/printed-circuit-board/1}{Roboflow}      \\
                Poker Cards                              & 53 & \textit{n/a} & 964   & 193   & 128   & 0.995 & 0.994   & -       & \href{https://app.roboflow.com/roboflow-100/pests-2xlvx/1}{Roboflow}                \\
                Number Ops                               & 15 & 28           & 4869  & 1636  & 623   & 0.991 & 0.991   & 0.055   & \href{https://app.roboflow.com/roboflow-100/cavity-rs0uf/1}{Roboflow}               \\



                Insects                                  & 10 & 0            & 696   & 199   & 100   & 0.855 & 0.798   & 0.024   & \href{https://app.roboflow.com/roboflow-100//insects-mytwu/1}{Roboflow}             \\
                Cotton                                   & 4  & 17           & 367   & 19    & 20    & 0.534 & 0.539   & 0.157   & \href{https://app.roboflow.com/roboflow-100/cotton-20xz5/1}{Roboflow}               \\
                Furniture                                & 3  & \textit{n/a} & 454   & 161   & 74    & 0.981 & 0.522   & 0.836   & \href{https://app.roboflow.com/roboflow-100/furniture-ngpea/1}{Roboflow}            \\
                Cable Damage                             & 2  & 2            & 919   & 256   & 134   & 0.904 & 0.838   & 0.006   & \href{https://app.roboflow.com/roboflow-100/cable-damage/1}{Roboflow}               \\
                Animals                                  & 10 & 12           & 700   & 200   & 100   & 0.76  & 0.0813  & 0.249   & \href{https://app.roboflow.com/roboflow-100/animals-ij5d2/1}{Roboflow}              \\


                Coins                                    & 4  & \textit{n/a} & 6121  & 1599  & 699   & 0.945 & 0.985   & 0.175   & \href{https://app.roboflow.com/roboflow-100//coins-1apki/1}{Roboflow}               \\
                Apples                                   & 2  & 0            & 489   & 178   & 30    & 0.775 & 0.798   & 0.271   & \href{https://app.roboflow.com/roboflow-100/apples-fvpl/1}{Roboflow}                \\
                People in Paintings                      & 1  & 5            & 634   & 194   & 81    & 0.548 & 0.657   & 0.168   & \href{https://app.roboflow.com/roboflow-100/people-in-paintings/1}{Roboflow}        \\
                Circuit Voltage                          & 6  & 11           & 92    & 25    & 15    & 0.794 & 0.343   & 0.009   & \href{https://app.roboflow.com/roboflow-100/circuit-voltages/1}{Roboflow}           \\
                Uno Deck                                 & 15 & \textit{n/a} & 6295  & 1798  & 899   & 0.994 & 0.994   & 0.013   & \href{https://app.roboflow.com/roboflow-100/uno-deck/1}{Roboflow}                   \\


                Grass Weeds                              & 1  & 105          & 1661  & 580   & 245   & 0.787 & 0.786   & 0.106   & \href{https://app.roboflow.com/roboflow-100/grass-weeds/1}{Roboflow}                \\
                Gauge                                    & 3  & 141          & 158   & 52    & 25    & 0.615 & 0.707   & 0.217   & \href{https://app.roboflow.com/roboflow-100/gauge-u2lwv/1}{Roboflow}                \\
                Sign Language                            & 26 & 0            & 504   & 144   & 72    & 0.95  & 0.893   & 0.006   & \href{https://app.roboflow.com/roboflow-100/sign-language-sokdr/1}{Roboflow}        \\
                Valentines Chocolate & 22 & 4            & 45    & 24    & 18    & 0.927 & 0.237   & 0.013   & \href{https://app.roboflow.com/roboflow-100/valentines-chocolate/1}{Roboflow}       \\
                Fish Market          & 21 & 252          & 13362 & 3558  & 1811  & 0.909 & -       & 0.013   & \href{https://app.roboflow.com/roboflow-100/fish-market-ggjso/1}{Roboflow}          \\



                Lettuce Pallets      & 5  & 168          & 1060  & 299   & 151   & 0.946 & 0.95    & 0.031   & \href{https://app.roboflow.com/roboflow-100/lettuce-pallets/1}{Roboflow}            \\
                Shark Teeth          & 4  & 154          & 191   & 53    & 36    & 0.951 & 0.659   & 0.025   & \href{https://app.roboflow.com/roboflow-100/shark-teeth-5atku/1}{Roboflow}          \\
                Bees                 & 1  & 163          & 5640  & 1604  & 836   & 0.903 & 0.691   & 0.009   & \href{https://app.roboflow.com/roboflow-100/bees-jt5in/1}{Roboflow}                 \\
                Sedimentary Features & 5  & 31           & 156   & 45    & 21    & 0.402 & 0.43    & 0       & \href{https://app.roboflow.com/roboflow-100/sedimentary-features-9eosf/1}{Roboflow} \\
                Currency             & 10 & 1            & 576   & 155   & 82    & 0.807 & 0.518   & 0.099   & \href{https://app.roboflow.com/roboflow-100/currency-v4f8j/1}{Roboflow}             \\


                Trail Camera         & 5  & 4            & 1060  & 299   & 151   & 0.96  & 0.968   & 0.512   & \href{https://app.roboflow.com/roboflow-100/trail-camera/1}{Roboflow}               \\
                Cell Towers          & 4  & 25           & 191   & 53    & 36    & 0.926 & 0.809   & 0.053   & \href{https://app.roboflow.com/roboflow-100/cell-towers/1}{Roboflow}                \\

                \hline
                \hline
            \end{tabular}
        }
    \end{center}

    \parbox{19.5cm}{\caption{The above table reports metadata about the 50 data-sets in the Real World category of RF100. It includes each data-set's name, number of classes, labeling hours spend by the original author, the train/validation/test split used, model's mAP@.50 value on the three bench marked models and the source link. In the labeling hours column, a zero value denotes that the dataset was annotated outside of the Roboflow app, and a \textit{n/a} value denotes that the dataset was created before Roboflow started keeping track of the labeling hours data.\label{table:two} }}
\end{table*}

